Neural Machine Translation for the Indigenous Languages of the Americas: An Introduction

Neural models have drastically advanced state of the art for machine translation (MT) between high-resource languages. Traditionally, these models rely on large amounts of training data, but many language pairs lack these resources. However, an important part of the languages in the world do not have this amount of data. Most languages from the Americas are among them, having a limited amount of parallel and monolingual data, if any. Here, we present an introduction to the interested reader to the basic challenges, concepts, and techniques that involve the creation of MT systems for these languages. Finally, we discuss the recent advances and findings and open questions, product of an increased interest of the NLP community in these languages.

==> table_and_citations.tex <==

\begin{table*}[th]
    \centering
    \begin{tabular}{|c|c|}
        \hline \bf Data & \bf Preprocessing \\\hline
        \begin{tabular}{@{}c@{}}
            Parallel data \S\ref{subsec:parallel_data}\\
            Bilingual dictionaries \S\ref{subsec:bilingual_dics_data}\\
            Monolingual text  \S\ref{subsec:monolingual_data}\\
            Linguistic annotated datasets \S\ref{subsec:linguistic_data}
        \end{tabular} 
        & 
         \begin{tabular}{@{}c@{}}
         Morphological segmentation  \S\ref{subsec:morph_seg}\\
         Probabilistic word segmentation \S\ref{subsec:prob_seg}
        \end{tabular}        
        
        \\\hline
        \bf Training algorithms & \bf Modeling \\\hline
        \begin{tabular}{@{}c@{}}
            Transfer Learning with pretraining  \S\ref{subsec:transferlearning}\\ 
            Pivoting  \S\ref{subsec:pivoting}\\
            Data augmentation  \S\ref{subsec:dataaugmentation}\\
            %Back-translation  \S\ref{subsec:backtranslation}\\
            Multilingual training  \S\ref{subsec:multilingual}\\
            Unsupervised Machine Translation \S\ref{subsec:umt}\\
            Training objectives and loss functions  \S\ref{subsec:mrt}\\
            Optimized hyperparameters \S\ref{subsec:optimize_params}
        \end{tabular} 
        &  
        \begin{tabular}{@{}c@{}}
            Integrating external knowledge to the model \S\ref{subsec:external_knowledge}\\
            Layers and architectures \S\ref{subsec:layers}
            
        \end{tabular} 
        \\\hline
    \end{tabular}
    \caption{A road map research directions in NMT for low resourced languages.}
    \label{tab:roadmap}
\end{table*}


\section{Data}
\label{sec:data}

\subsection{Parallel data}
\label{subsec:parallel_data}

\cite{mccarthy-EtAl:2020:LREC1} % Bible
% TODO Add other bible corpora
\cite{agic-vulic-2019-jw300} % jw300
\cite{guzman2019flores} % Flores dataset
% Add bilingual dictionary
\cite{mayer2014creating} % Creating bible corpora
\cite{tiedemann2016opus} % Opus dataset

\subsection{Bilingual dictionaries}
\label{subsec:bilingual_dics_data}

\cite{kamholz2014panlex} % PanLex project
\cite{schwenk2019wikimatrix} % Bitext matrix on 1620 languages
\subsection{Monolingual text}
\label{subsec:monolingual_data}
\cite{ortizsuarez:hal-02148693} %Oscar
\cite{wiki} % Wikipedia
\subsection{Linguistic annotated datasets}
\label{subsec:linguistic_data}

\section{Preprocessing}
\label{sec:preprocessing}
\cite{vania-lopez-2017-characters} % Analsys about usage of different inputs for NLP

\subsection{Morphological segmentation}

Most used segmentation tools: \cite{creutz-2003-unsupervised} % Morphesor
\cite{smit-etal-2014-morfessor} % Morphesor
\cite{ruokolainen2013supervised} % CRF
\cite{pan2020morphological} % Hybrid of BPE and morphological segmentation.
\cite{gronroos2014morfessor} % Flatcat
\cite{wu2016google} % Words + characters

Applications: \label{subsec:morph_seg} \cite{rikters2018training} \cite{zhou2019low} 
\cite{pan-etal-2020-multi}
% On multi-task (translaton + stemming)
% Also shows that mophological segmentation is better pre processing for agglutinative languages than BPE

\subsection{Probabilistic word segmentation}

\cite{gage1994new} % Original BPE with out NLP application
\cite{sennrich-etal-2016-neural} % BPE
\cite{kudo2018subword} % Sentence piece Unigram language model
\cite{sperr-etal-2013-letter} % Wors segment into character trigrams
\label{subsec:prob_seg}
\subsection{Parallel data filtering and mining}
\label{subsec:cleaning_data}

\cite{koehn2019findings} %WMT corpus filtering shared task TODO: Should I add all systems from the Shared Task?
\cite{hangya2019unsupervised} % Mining




\section{Training algorithms}
\label{sec:trining}

\subsection{Transfer learning with pretraining}
\label{subsec:transferlearning}
%DOBE
\cite{gulcehre2015using} % pretrained LM as decoder in NMT
\cite{zopf-etal-2016-beyond} % Pretraining on high resource language and fine tune on low resource language TODO: is it zoph2016transfer?
\cite{nguyen2017transfer} % Usage of related languages
\cite{baziotis2020language} % LM as priors at decoding time
\cite{neubig2018rapid} % Avoid over fitting with fine-tuning
\cite{edunov2019pre} % use ELMO
\cite{conneau2019cross} % XLM
\cite{song2019mass} % MASS
\cite{lewis2019bart} % BART
\cite{liu2020multilingual} % mBART
\cite{li2020data} % BART with gaussian prior objective
\cite{brown2020language} % Improve in Zero shot
\cite{song2020pre} % TODO. Read again
\cite{zhu2020incorporating} % BERT into NMT
\cite{aji-etal-2020-neural} % What does transfer learning transfer? 
\cite{wang2019denoising} % Should go to TODO!!!
% transfer just the Embedding layer does not help
% Embedding layer + rest is the best
% joint embeddings are better
\subsection{Pivoting}
\label{subsec:pivoting}

\cite{wu-wang-2007-pivot} % SMT pivoting
\cite{cohn-lapata-2007-machine} % SMT pivoting
\cite{utiyama2007comparison} % SMT pivoting
\cite{zheng-etal-2017-joint} % Joint training TODO: check
\cite{cheng2019joint} % Joint Training TODO: check
\cite{ahmadnia2019augmenting} % round-trip training TODO: check
\cite{pourdamghani2019neighbors} % Application: relanted languages
\cite{lakew2018improving}  % multilingual zero shot
\cite{leng2019unsupervised} % (see \S\ref{subsec:umt}) %Improving UMT Distante languages

\subsection{Data augmentation}
\label{subsec:dataaugmentation}
%DONE 

\cite{fadaee2017data} % Replacing frequent words by low-requency  ones
\cite{zhu2019soft} % Soft words using hidden states of a LM
\cite{kobayashi2018contextual} %General augmentation paper, that uses a conditioned LM for contextual augmentation.
\cite{wu2019conditional} %Use a conditional BERT for agumentation
\cite{hu2019learning} %Joint learning of MT and LM

%\subsection{Back-translation}
\label{subsec:backtranslation}

\cite{sennrich2016improving} % Back translation paper
\cite{hoang2018iterative} % Iterative back translation. Importance of first translation system.
\cite{edunov2019evaluation} % improving only metric with translationese
\cite{gu2019improved} % Zero-shot machine NMT with BT
\cite{edunov2018understanding} % Sampling at decoding time of BT helps in high resource settings, but beam is better for low
\cite{caswell2019tagged} % BT improves when adding a special symbol to the synthetic data
\cite{abdulmumin2019tag} % Initial training with BT data and then finetuning with natural data.


\cite{soto-etal-2020-selecting}
% Improving backtranslation
% Combining generated text from multiple systems (SMT, RNN, Transformers) is the best.
% They propose re-ranking outputs based on Feature decay algorithm
\cite{marie-etal-2020-tagged}
% Analysis of tagged BT


\subsection{Multilingual training}
\label{subsec:multilingual}
%DONE

\cite{johnson2017google} % Google multilingual
\cite{blackwood2018multilingual} % Shareing all parameters with exception of attention
\cite{sachan2018parameter} % Parameter sharing for one to many, transformers 
\cite{lu2018neural} % prose a shared layer for interlingua information  (see Modeling)
\cite{zaremoodi2018adaptive} % Routing network  ( see Modeling)
\cite{platanios2018contextual} % Contextual parameter generator (see modeling)
\cite{arivazhagan2019missing} % representational invariance training  (see: Modeling)
\cite{neubig2018rapid} % 58 languages
\cite{arivazhagan2019massively} % 102 languages
\cite{tiedemann2018emerging} % On 900 languages of the bible. Find interlingua representation.
\cite{malaviya2017learning} % Predicts typology for from interlingua representations. Uses the bible 
\cite{tan2019study} % survey
\cite{dabre2019survey} % survey
\cite{zhang2020improving} % explore problems TODO: check again
\cite{aharoni2019massively} % 102 languages  and performance drops with many languages.
%\cite{zhang2020improving} % language aware input layer (See Modeling)
%\cite{zhang-etal-2019-improving} % online back-translation (See Modeling)
\cite{wang-etal-2020-balancing}
% Problem with balanced data for multilingual training
% learn data selection
% DDS and reinforcement learning for the scorer
% On TED dataset (two samples)
\cite{siddhant-etal-2020-leveraging}
% Merge multilingual training and monolingual pretraining


\subsection{Unsupervised Machine Translation}
\label{subsec:umt}


Bilingual word embeddings: \cite{artetxe-etal-2017-learning} \cite{zou2013bilingual}
UMT
\cite{lample2017unsupervised} , see \S\ref{sec:modeling}% Auto encoder with adversarial training
\cite{conneau2017word} % Bilingual word embeddings are not isomorphic for different typologies
\cite{artetxe2018unsupervised} % Auto encoders with shared encoding space and separate decoders for each language
\cite{sogaard2018limitations} % Limitations of UMT
\cite{marie2019nict} % Combining SMT and NMT
\cite{artetxe2019effective} %with SMT
\cite{ren2019unsupervised} % Regularizing with SMT
\cite{stojanovski2019lmu} % Using masked language model and denoising  autoencoding
\cite{vulic-etal-2019-really} % Semi-supervised bilingual word embeddings help to improve isomprhism
\cite{leng2019unsupervised} % Including pivoting to avoid distant language pairs
\cite{liu2019incorporating} % combine word-level and sub-word level embeddings
\cite{su2019unsupervised} % mutli modal UMT
\cite{sun2020robust} % Adversarial training
\cite{barrault2019findings} % shared features with subtask
\cite{vulic2020all} % with reduced data size non isomorphic
% \cite{nooralahzadeh2020zero} % performance deteriorate when mismatch of domains TODO: WRONG CITATION! Try to find the correct one
\cite{artetxe2020call} % Non realistic sceanrio for UMT

% Applications
\cite{zhang2018style} % style transfer

\subsection{Training objectives and loss functions}
\label{subsec:mrt}

\cite{zhang-etal-2019-improving} % online back-translation 
\cite{wieting2019beyond} % For back translation 
\cite{arivazhagan2019missing} % representational invariance training  (see: Modeling?)
\cite{li2020data} % MASS with gaussian prior objective TODO: classify correctly
\cite{lample2017unsupervised} , see \S\ref{sec:umt}% UMT with Auto encoder with adversarial training
\cite{pan-etal-2020-multi}, see \S\ref{sec:preprocessing}
%Multitask learning, performing translation and steam prediction for agglutinative languages


\subsection{Optimized hyperparameters}
\label{subsec:optimize_params}
\cite{sennrich2019revisiting} %Hyper parameter tuning
\cite{guzman2019flores}
\cite{biljon2020} % Best transformer depth for low-resource languages

\section{Modeling}

\label{sec:modeling}


\subsection{Integrating external knowledge into the model}
\label{subsec:external_knowledge}

\cite{du2016using} % BabelNet TODO: How and classify
\cite{moussallem2018machine,moussallem2019augmenting} % knowledge graphs TODO: How and classify
\cite{annervaz2018learning} % entity linking TODO: How and classify
\cite{armengol2020enriching} % linguistic features TODO: how and classify (maybe preprocessing)


\subsection{Layers and architectures}
\label{subsec:layers}

\cite{miceli2017deep} %BiDeep RNN 
\cite{szegedy2016rethinking} % label smoothing 
\cite{sennrich2016edinburgh} % Word dropout 
\cite{ba2016layer} % Normalization layer 
\cite{nguyen-etal-2015-improving} % Lexical model
\cite{press2017using} % Tied embeddings
\cite{zhang2020improving} % language aware input layer (see multilingual)
\cite{wang2019denoising} % pointer network layer 
\cite{zaremoodi2018adaptive} % Routing network 
\cite{platanios2018contextual} % Contextual parameter generator (see multilingual)
\cite{lu2018neural} % prose a shared layer for interlingua information  (see multilingual)
